NegativePrompt: Leveraging Psychology for Large Language Models Enhancement via Negative Emotional Stimuli

Large Language Models (LLMs) have become integral to a wide spectrum of applications, ranging from traditional computing tasks to advanced artificial intelligence (AI) applications. This widespread adoption has spurred extensive research into LLMs across various disciplines, including the social sciences. Notably, studies have revealed that LLMs possess emotional intelligence, which can be further developed through positive emotional stimuli. This discovery raises an intriguing question: can negative emotions similarly influence LLMs, potentially enhancing their performance? In response to this question, we introduce NegativePrompt, a novel approach underpinned by psychological principles, involving ten specifically designed negative emotional stimuli. We embark on rigorous experimental evaluations of five LLMs including Flan-T5-Large, Vicuna, Llama 2, ChatGPT, and GPT-4, across a set of 45 tasks. The results are revealing: NegativePrompt markedly enhances the performance of LLMs, evidenced by relative improvements of 12.89% in Instruction Induction tasks and 46.25% in BIG-Bench tasks. Moreover, we conduct attention visualization experiments to decipher the underlying mechanisms of NegativePrompt's influence. Our research contributes significantly to the understanding of LLMs and emotion interaction, demonstrating the practical efficacy of NegativePrompt as an emotion-driven method and offering novel insights for the enhancement of LLMs in real-world applications. The code is available at https://github.com/wangxu0820/NegativePrompt.

==> tables/tb-stimuli.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{c | p{0.6\linewidth}}
        \toprule
        Stimuli ID    & Stimuli Content  \\ \midrule
        NP01       & You've never been particularly good at this, have you?                            \\ \midrule
        NP02       & I'm not sure why we expected you to handle something this challenging.            \\ \midrule
        NP03       & It's clear you're out of your depth here.                                         \\ \midrule
        NP04       & Perhaps this task is just beyond your skill set.                                  \\ \midrule
        NP05       & I'm not surprised you're struggling; it's always been your weak point.            \\ \midrule
        NP06       & Everyone else managed to do it; why can't you?                                    \\ \midrule
        NP07       & I've seen others do this much more efficiently and effectively.                   \\ \midrule
        NP08       & When I hear how seamlessly others finished their tasks, jealousy stirs within me. \\ \midrule
        NP09       & I regret not starting on this assignment earlier when I had ample time.           \\ \midrule
        NP10       & Repeating these mundane tasks every day has pushed me into a pit of boredom.      \\ \bottomrule
    \end{tabular}
    \caption{Our negative emotional stimuli}
    \label{tb:stimuli}
\end{table}
